Graph neural network for 3D classification of ambiguities and optical crosstalk in scintillator-based neutrino detectors

Deep learning tools are being used extensively in high energy physics and are becoming central in the reconstruction of neutrino interactions in particle detectors. In this work, we report on the performance of a graph neural network in assisting with particle flow event reconstruction. The three-dimensional reconstruction of particle tracks produced in neutrino interactions can be subject to ambiguities due to high multiplicity signatures in the detector or leakage of signal between neighboring active detector volumes. Graph neural networks potentially have the capability of identifying all these features to boost the reconstruction performance. As an example case study, we tested a graph neural network, inspired by the GraphSAGE algorithm, on a novel 3D-granular plastic-scintillator detector, that will be used to upgrade the near detector of the T2K experiment. The developed neural network has been trained and tested on diverse neutrino interaction samples, showing very promising results: the classification of particle track voxels produced in the detector can be done with efficiencies and purities of 94-96% per event and most of the ambiguities can be identified and rejected, while being robust against systematic effects.

==> Unused/movitation_previous_order.tex <==
\section{Motivation}
\label{sec:motivation}

Finely segmented scintillator detectors consist of a 3D array of plastic scintillator cubes read-out in three orthogonal 2D projections. Charged particles traversing the cubes produce scintillation light, giving rise to signals in each of the three 2D views, depicted in Fig.~\ref{fig:projections}. In terms of event reconstruction the scintillator cubes with detected signals are refered to as \emph{voxels}. To reconstruct the neutrino interactions in three dimensions, the three 2D views must be matched together, as shown in Fig.~\ref{fig:3D}. However, ambiguities in the matching process can give rise to 3D \emph{ghost} voxels (apparent signals in a cube that was not traversed by a charged particle), shown in Fig.~\ref{fig:ghost}. Furthermore, as seen in Fig.~\ref{fig:xtalk}, light-leakage between neighbouring cubes can create \emph{crosstalk} signals.\\
\indent To accurately reconstruct neutrino interactions in these detectors it is crucial to be able to identify the energy deposit in each scintillator cube (classify each voxel) as one of the three types:
\begin{itemize}
    \item \textbf{Track}: a real energy deposit from a charged particle, henceforth referred to as \emph{track} signals.
    \item \textbf{Crosstalk}: a real energy deposit from light-leakage.
    \item \textbf{Ghost}: fake signal coming from the ambiguity when matching the three 2D views into 3D.
\end{itemize}
Figure~\ref{fig:goal} shows the three types of voxels using truth information after 3D matching has been performed for an example neutrino interaction. Once these voxels can be classified, the ghost signals can be removed before the full event reconstruction proceeds, while simultaneously cleaning the particle tracks of crosstalk.
\begin{figure}[htb]
    \centering
%    \begin{tabular}{cc}
		\includegraphics[width=0.8\linewidth]{plots/ghost.pdf}
%	\end{tabular}
	\caption{Example of ghost voxel appearance. Seeing only the charge deposition coming from the three fibers, a voxel could either have deposited charge (then it is a track voxel) or just appear while matching coordinates of the fibers, becoming a non-physical ghost voxel.}
    \label{fig:ghost}
\end{figure}
\begin{figure}[htb]
    \centering
%    \begin{tabular}{cc}
		%\includegraphics[width=0.99\linewidth]{plots/xtalk_sketch.pdf}
		\includegraphics[width=0.99\linewidth]{plots/xtalk_sketch-2.png}
%	\end{tabular}
	\caption{Sketch of the signal generation, fiber transport and signal detection processes highlighting the production of optical crosstalk signals.}
    \label{fig:xtalk}
\end{figure}

In this article, we represent the scintillator cubes with detected signals as points in a graph and classify the signals using a deep learning technique based on a GNN. The abstract data representation provided by graphs makes this method very versatile and applicable to any experiment where the output data from the detector elements can be represented as a list of features with arbitrary dimensionality. Here, we consider the Super Fine-Grained Detector (SuperFGD)~\cite{Abe:2019whr} as a specific case-study. The detector contains 192$\times$56$\times$184 plastic scintillator cubes, each 1$\times$1$\times$1\,cm$^3$ in size. The cubes are intersected by three orthogonal wavelength-shifting (WLS) fibers that transport the scintillation light to silicon photomultipliers (SiPMs), as illustrated in Fig.~\ref{fig:cube3d}. A full description of the SuperFGD is given in Ref.~\cite{Abe:2019whr}.
\begin{figure}[hbt]
    \centering
		\includegraphics[width=0.7\linewidth]{plots/CubeGEANT4.png}
	\caption{Geometry of a single SuperFGD cube.}
    \label{fig:cube3d}
\end{figure}

%\indent In this article, the SuperFGD is used as a specific case-study. The detector consists of a large array of scintillator cubes and neutrino interactions are imaged in three 2D planes, which are matched together to form a 3D voxelised representation of the data. Each voxel can be empty, or have one of three types of signal: a real energy deposit from a charged particle track, an energy deposit caused by light-leakage (cross-talk) from a neighbouring scintillator cube, or a fake signal (henceforth called \emph{ghosts}) caused by ambiguities in the 3D matching procedure.\\
%\indent To accurately reconstruct neutrino interactions it is critical to be able to classify voxels as one of the three types: track, cross-talk or ghost. In the technique presented here, each voxel containing an energy deposit is represented as a point in a graph and classified using a deep learning technique called a Graph Neural Network (GNN)~\cite{SperdutiFirstGNN}. The abstract data representation provided by graphs makes this method very versatile and applicable to any experiment where the output data from the detector elements can be represented as a list of features with arbitrary dimensionality. 

%%%% Original paragraphs from Cesar %%%%
%In the later case, optical cross-talk among neighbor detector cells and matching ambiguities from 2D to 3D are potential nuisances for this technology.
%The first compromising the fine granularity and the second generating fake signals. The high variety of neutrino event signals does the nuisance removal highly complex via standard methods making Neural Network approaches suitable candidates for this classification problem. In this study a new approach is presented. Each fired cell is translated into a voxel with a set of associated properties and connected to other neighbor voxels to form a Graph. Under this picture a Graph Neural Network is trained to classify each individual voxel as a type of signal.

%Remarkably, this method can be used to classify signals in a very wide range of HEP detectors and applications thanks to the abstraction of the Graph. Any segmented detector using strips, pixels, bars or cells, provides output data of arbitrary dimensionality that can be translated into a graph and classified as presented here. If the signal and the background are non-trivially correlated this method provides a possible solution to efficiently separate them.

==> Unused/temp.tex <==

%OLD EFF/PUR TABLES

\begin{table*}[htb]
    \centering
    %\setlength{\tabcolsep}{6pt}
    \begin{tabular}{l|lccc|lccc}
    \hline \hline
    \rule{0pt}{9pt}& \multicolumn{4}{c|}{\textbf{GENIE Training}} & \multicolumn{4}{c}{\textbf{Pbomb Training}}\\
    \hline
    \rule{0pt}{9pt}\multirowcell{3}{\textbf{GENIE}\\\textbf{Testing}} & & Track & Crosstalk & Ghost & & Track & Crosstalk & Ghost\\ 
    &Efficiency & 94\% & 94\% & 88\% & Efficiency & 94\% & 93\% & 88\%\\
    &Purity & 96\% & 91\% & 92\% & Purity & 95\% & 91\% & 91\%\\
    \hline
    \rule{0pt}{9pt}\multirowcell{3}{\textbf{Pbomb}\\\textbf{Testing}} & & Track & Crosstalk & Ghost & & Track & Crosstalk & Ghost\\ 
    &Efficiency & 94\% & 94\% & 87\% & Efficiency & 95\% & 93\% & 88\%\\
    &Purity & 96\% & 90\% & 92\% & Purity & 96\% & 91\% & 92\%\\
    \hline \hline
    \end{tabular}
    \caption{Mean efficiencies and purities of voxel classification, per event.}
    \label{tab:eff&pur_evt}
\end{table*}


\begin{table*}[htb]
    \centering
    %\setlength{\tabcolsep}{6pt}
    \begin{tabular}{l|lccc|lccc}
    \hline \hline
    \rule{0pt}{9pt} & \multicolumn{4}{c|}{\textbf{GENIE Training}} & \multicolumn{4}{c}{\textbf{Pbomb Training}}\\
    \hline
    \rule{0pt}{9pt}\multirowcell{3}{\textbf{GENIE}\\\textbf{Testing}} & & Track & Crosstalk & Ghost & & Track & Crosstalk & Ghost\\ 
    &Efficiency & 93\% & 90\% & 84\% & Efficiency & 93\% & 89\% & 80\%\\
    &Purity & 93\% & 87\% & 91\% & Purity & 91\% & 86\% & 89\%\\
    \hline
    \rule{0pt}{9pt}\multirowcell{3}{\textbf{Pbomb}\\\textbf{Testing}} & & Track & Crosstalk & Ghost & & Track & Crosstalk & Ghost\\ 
    &Efficiency & 94\% & 93\% & 87\% & Efficiency & 95\% & 93\% & 88\%\\
    &Purity & 95\% & 90\% & 92\% & Purity & 95\% & 91\% & 92\%\\
    \hline \hline
    \end{tabular}
    \caption{Mean efficiencies and purities of voxel classification, per voxel.}
    \label{tab:eff&pur_vox}
\end{table*}



%old xTalk table
\begin{table*}[htb]
    \centering
    \begin{tabular}{lccc|lccc|lccc}
    \hline \hline
    \multicolumn{4}{c|}{\textbf{Crosstalk 2.7\% (nominal)}} &
    \multicolumn{4}{c|}{\textbf{Crosstalk 2\%}} &
    \multicolumn{4}{c}{\textbf{Crosstalk 5\%}}\\
    \hline
     & Track & Crosstalk & Ghost & & Track & Crosstalk & Ghost  & & Track & Crosstalk & Ghost\\ 
    Efficiency & 93\% & 90\% & 84\%  &Efficiency & 92\% & 89\% & 81\% & Efficiency & 94\% & 89\% & 88\%\\
    Purity & 92\% & 87\% & 91\% &Purity & 94\% & 83\% & 89\% & Purity & 86\% & 91\% & 93\%\\
    \hline \hline
    \end{tabular}
    \caption{Mean efficiencies and purities of voxel classification, per voxel, for different crosstalk values, i.e. 2.7\% (nominal) 2\% and 5\%. The GNN was trained with GENIE training samples with nominal crosstalk and tested on the same GENIE sample with different crosstalk values to study its robustness.}
    \label{tab:eff&pur_evt_otherXtalk}
\end{table*}

==> old/old_motivation.tex <==

\section{Motivation}
\label{sec:motivation}

Since 1999 a series of neutrino oscillation experiments provided a deep insight into the nature of neutrinos~\cite{oscSuperK,oscSNO,oscKamland,oscK2K,oscDayaBay,MINOSFinal3Flav,Acero:2019ksn,Abe:2019vii}. A number of these experiments are long-baseline neutrino oscillation experiments with the following basic concept:
%The basic concept of this kind of experiment is the following: 
%a beam of protons is collided with a graphite target and the outgoing pions and kaons are, depending 
%on the charge of the particle, focused or defocused  using a system of magnetic horns.
%The produced beam of mesons traverses a about 100 m long tunnel in which the particles decay producing
%in this way a beam of neutrinos or anti-neutrinos. 
two detectors are used to characterize a beam of (anti-)neutrinos: one, the near detector, is located a few hundred meters away from the target and characterizes
the original beam composition, while the second one, the far detector, is located several hundred kilometres away and allows to measure the beam composition after neutrino flavor oscillations.

The energy of the neutrinos ranges from a few tens of MeV up to several GeV. When the neutrino interacts
with the detector material, charged particles can be produced which are detected while traversing
the detector. For neutrino energies of a few hundred MeV, the dominant physics process is the charged-current quasi-elastic interaction with mainly a single charged lepton in the final state. For higher energies
$\Delta$ resonances and deep inelastic interactions gain relevance leading to far more complex hadronic final 
states with multiple protons and pions leaving the interaction vertex over a $4\pi$ solid angle.
%Therefore, to minimize the systematic uncertainties and maximize the sensitivity of current and future
%oscillation experiments, it is necessary that both, near and far detector, provide a $4\pi$ coverage for the outgoing particles.\\
\textcolor{blue}{Davide: Do we need details about the neutrino interaction modes ? What about just saying how the final state looks like. Also, I would move after introducing CP violation at T2K.}

\textcolor{blue}{Davide: I would add a general introduction to next generation neutrino detectors, i.e. LAr and sFGD, as well as physics goal without too many details about T2K}
\textcolor{green}{Cesar: I agree. Who does it?}

The T2K collaboration recently published indications for CP violations in the leptonic
sector~\cite{Abe:2019vii}. To improve the sensitivity of the experiment further, the collaboration proposed the
T2K-II phase which includes an upgrade of the beam power from 500 kW to 1.3\,MW~\cite{Abe:2019fux} and an upgrade of 
its near detector, doubling its mass and achieving a $4\pi$ coverage for the outgoing particles \cite{Abe:2019whr} aiming for a reduction of systematic uncertainties limiting the current results.

\textcolor{blue}{Davide: What about introducing the need for machine learning techniques here ? Then we can justify it given the complexity of neutrino interactions we want to reconstruct.}

\textcolor{blue}{Davide: I would introduce sFGD as an example for our study, like ``We take the sFGD detector as an example study for '' }

The key element of the near detector upgrade is the Super-Fine Grained Detector (SFGD), a scintillator tracker based on a novel concept \cite{Blondel_2018}. While classical scintillator tracker
are based on bars or fibers, the SFGD consists of scintillating cubes which are optically isolated from each other. Each of the cubes is crossed along the axes by three wavelength shifting fibers. Each of the fibres is readout single sided by an SiPM providing in this way three orthogonal 2D views of the interactions within the detector. A 3D image can be obtained from the combination of the 2D views in which each 3D hit, voxel, 
corresponds to one of the cubes in the detector. An almost identical detector, called the 3DST, is planned as part of the next-generation Deep Underground Neutrino Experiment (DUNE) Near Detector suite~\cite{3DST_ICHEP,duneTDR}. However, the SFGD will be built and operational on a shorter timescale than the 3DST so in this article we focus specifically on the SFGD.
\textcolor{blue}{Davide: Reduce description of sFGD detector and move details to ``methodology'' section\\}
\textcolor{blue}{Davide: we should mention somewhere here that sFGD has 2M cubes, i.e. voxels, because we refer to this number later in the text.}
For the correct reconstruction of the physics event, it is necessary to classify each voxel either as a track, cross-talk or ghost voxel. A track voxel corresponds to a cube through which a charged particle has directly crossed. Cross-talk voxels have their origin in the leakage of light from a track cube to a neighboring cube since the optical isolating layer of the cubes is not 100\% opaque; in the case of
the SFGD the leakage is of the order of a few percent.

While these two types of voxels are physical, a third class, called ghosts, is an artefact of the 3D reconstruction based on three 2D views. This kind of artefact is a serious problem for the performance of the detector if not identified as such since they might lead to the reconstruction of nonphysical tracks and therefore affects the measured track multiplicity in the final state of the neutrino interaction.

In the following, a classification method for the voxels based on a Graphical Neural Network (GNN) is presented and compared with a traditional cut-based method.% method based on classical cuts.
\textcolor{blue}{Davide: I would not emphasize too much the comparison with cut-based methods since we will probably have only a short paragraph about it.}

==> old/old_motivation_new.tex <==

\section{Introduction}
\label{sec:introduction}

%\textcolor{blue}{Davide\&Cesar: emphasize the potential of GNN for particle-flow reconstruction and provide references / examples from LHC applications (e.g. calorimeters, etc.)//
%Leigh: we give these examples in the neural networks section, so maybe we just be generic here.}

Since 1999 a series of neutrino oscillation experiments have provided deep insight into the nature of neutrinos~\cite{oscSuperK,oscSNO,oscKamland,oscK2K,oscDayaBay,MINOSFinal3Flav,Acero:2019ksn,Abe:2019vii}. A number of these experiments are long-baseline neutrino oscillation experiments that use
%The basic concept of this kind of experiment is the following: 
%a beam of protons is collided with a graphite target and the outgoing pions and kaons are, depending 
%on the charge of the particle, focused or defocused  using a system of magnetic horns.
%The produced beam of mesons traverses a about 100 m long tunnel in which the particles decay producing
%in this way a beam of neutrinos or anti-neutrinos. 
two detectors to characterize a beam of (anti-)neutrinos: one, the near detector, is located a few hundred meters away from the target and measures the original beam composition, while the second one, the far detector, is located several hundred kilometres away and allows for the determination of the beam composition after neutrino flavor oscillations.

The energy of the neutrinos in these beams ranges from a few tens of MeV up to several GeV. Charged particles can be produced when neutrinos interact with the detector material, which are detected while traversing the detector leaving a signal used to reconstruct the neutrino properties. In general, the larger the energy transferred from the neutrino to the nucleus the larger the number of particles and particle types produced in the final state. Modelling the nuclear interactions in the target nucleus is highly complex, particularly for high energy transfers where the hadronic component of the interaction is more important. As a result, current long-baseline neutrino oscillation experiments mostly work with interactions with low particle multiplicity. This situation however, is expected to change in the coming years. On one hand, the statistical and systematic uncertainties of current experiments have decreased significantly over recent years such that neutrino-nucleus modelling is becoming a dominant source of uncertainty~\cite{NOvA:2018gge,Abe:2019vii}. On the other hand, future experiments like DUNE~\cite{duneTDR} will use a broad-band energy neutrino beam expecting most of the neutrino interactions to have a high energy transfer to the nucleus. 

As a result, in recent years the neutrino physics community have turned their attention to measuring neutrino-nucleus interaction cross-sections for different ranges of energies and target materials \cite{Tanabashi:2018oca} as a way to constrain the oscillation uncertainties while providing new measurements to further develop the interaction models. In parallel, a new generation of neutrino detectors is under development. A key goal for these detectors is to resolve and reliably identify shorter particle tracks even in very complex interactions. To achieve this, two main detector technologies stand out: one is based on Liquid Argon Time-Projection-Chambers (LArTPCs)~\cite{Rubbia:1977zz} %,Amerio:2004ze,Anderson:2011ce,Acciarri:2016smi,Abi:2017aow} %[\textcolor{purple}{e.g. ArgoNeuT, microBooNE, Aridane, DUNE single phase, DUNE dual phase}]  [\textcolor{red}{references}]
and the other is based on finely segmented plastic scintillators~\cite{Blondel_2018}, such as the SuperFGD~\cite{Abe:2019whr} and the 3DST~\cite{3DST_ICHEP} detectors that will form part of the near detectors for T2K and, possibly, DUNE, respectively.\\
%Both approaches rely, in different ways, on reconstructing 3D information out of 2D projected information. In the case of LArTPCs, time of arrival is used to unfold the third spatial coordinate using the drift velocity. In the case of the new scintillator-based detectors, three orthogonal 2D views are matched to obtain the 3D information. 
% Thoughts from Leigh... I made this paragraph more specific to explain a little more about the SuperFGD to point out we are using it as a concrete example and introduce the terms used throughout the paper
\indent For the latter, these finely segmented scintillator detectors consist of a 3D array of plastic scintillator cubes read-out in three orthogonal 2D projections. Charged particles traversing the cubes produce scintillation light, giving rise to signals in each of the three 2D views. To reconstruct the neutrino interactions in three dimensions, the three 2D views must be matched together, but ambiguities in the matching process can give rise to 3D \emph{ghost} hits (apparent signals in a cube that was not traversed by a charged particle). Furthermore, light-leakage between neighbouring cubes can create \emph{crosstalk} signals. To accurately reconstruct neutrino interactions in these detectors it is crucial to be able to identify the energy deposit in each scintillator cube as one of the three types: a real energy deposit from a charged particle, henceforth refered to as \emph{track} signals; a real energy deposit from crosstalk; or a fake ghost signal. The ghost signals can then be removed before the full event reconstruction proceeds.\\
\indent In this article, we represent the scintillator cubes with detected signals as points in a graph and classify the signals using a deep learning technique based on a Graph Neural Network (GNN)~\cite{SperdutiFirstGNN}. The abstract data representation provided by graphs makes this method very versatile and applicable to any experiment where the output data from the detector elements can be represented as a list of features with arbitrary dimensionality. Here, we consider the SuperFGD as a specific case-study. The detector contains 192$\times$56$\times$184 plastic scintillator cubes, each 1$\times$1$\times$1\,cm$^3$ in size. The cubes are intersected by three orthogonal wavelength-shifting (WLS) fibers that transport the scintillation light to silicon photomultipliers (SiPMs), as illustrated in Fig.~\ref{fig:cube3d}. A full description of the SuperFGD is given in Ref.~\cite{Abe:2019whr}.
\begin{figure}[hbt]
    \centering
%    \begin{tabular}{cc}
		\includegraphics[width=0.7\linewidth]{plots/CubeGEANT4.png}
%	\end{tabular}
	\caption{Geometry of a single SuperFGD cube.}
    \label{fig:cube3d}
\end{figure}\\
\indent The article proceeds in the following way: Sec.~\ref{sec:introNN} introduces deep learning techniques and Sec.~\ref{sec:graphsage} details the specific GNN algorithm used. The simulated data samples and GNN training is discussed in Sec.~\ref{sec:methodology}. Results and a study of systematic uncertainties are given in Sections~\ref{sec:results} and~\ref{sec:systematics}, respectively, followed by concluding remarks in Sec.~\ref{sec:conclusions}.

%\indent In this article, the SuperFGD is used as a specific case-study. The detector consists of a large array of scintillator cubes and neutrino interactions are imaged in three 2D planes, which are matched together to form a 3D voxelised representation of the data. Each voxel can be empty, or have one of three types of signal: a real energy deposit from a charged particle track, an energy deposit caused by light-leakage (cross-talk) from a neighbouring scintillator cube, or a fake signal (henceforth called \emph{ghosts}) caused by ambiguities in the 3D matching procedure.\\
%\indent To accurately reconstruct neutrino interactions it is critical to be able to classify voxels as one of the three types: track, cross-talk or ghost. In the technique presented here, each voxel containing an energy deposit is represented as a point in a graph and classified using a deep learning technique called a Graph Neural Network (GNN)~\cite{SperdutiFirstGNN}. The abstract data representation provided by graphs makes this method very versatile and applicable to any experiment where the output data from the detector elements can be represented as a list of features with arbitrary dimensionality. 

%%%% Original paragraphs from Cesar %%%%
%In the later case, optical cross-talk among neighbor detector cells and matching ambiguities from 2D to 3D are potential nuisances for this technology.
%The first compromising the fine granularity and the second generating fake signals. The high variety of neutrino event signals does the nuisance removal highly complex via standard methods making Neural Network approaches suitable candidates for this classification problem. In this study a new approach is presented. Each fired cell is translated into a voxel with a set of associated properties and connected to other neighbor voxels to form a Graph. Under this picture a Graph Neural Network is trained to classify each individual voxel as a type of signal.

%Remarkably, this method can be used to classify signals in a very wide range of HEP detectors and applications thanks to the abstraction of the Graph. Any segmented detector using strips, pixels, bars or cells, provides output data of arbitrary dimensionality that can be translated into a graph and classified as presented here. If the signal and the background are non-trivially correlated this method provides a possible solution to efficiently separate them.


==> old/section4.tex <==
\section{Detector concept and problem description}
\label{sec:training-sample}


\textcolor{blue}{Cesar: I have written this section 4 before section 5 on demand by Sebastian and Saul. However reading the whole paper my impressions is that this 4th section can be removed completly, simply moving Fig2 to Detector geometry in section 5. The motivations for SuperFGD and the classification problem I believe are clearly enough stated in the motivation (and if something is missing doesn't need a whole section, it can be added to section 1). The only 'relevant' information that this section 4 provides is a bit more details on SuperFGD geometry (that again can be migrated to detector geometry in section 5. On top of this in my opinion this section is too much T2K-ish.}\\
In order to measure neutrino interactions a detector is exposed to a source of neutrinos such that neutrinos interacting in the detector material generate a set of outgoing tracks which leave signals in the detector while they propagate. Each detector concept works on a specific approach to collect these signals and to extract out of them as much information from the original neutrino as possible.

In the case of scintillator trackers used in neutrino detectors [NoVa \textcolor{red}{(NOvA technically uses liquid scintillator, Cesar: I have to check!! - Leigh: It uses plastic "tubes" filled with liquid, but it is effectively two planes of long scintillator)}, MINOS, ND280...] the usual approach has been to use long bars of scintillator material. The scintillation light produced by tracks propagating in the bar is collected and read in one end. Sets of planes rotated 90 degrees are stacked such that two complementary planes offer very good tracking capabilities along one axis, the efficiency however, drops at high angle. This is a relevant problem for neutrino oscillation experiments contributing substantially to the systematic uncertainty of the oscillation measurements given that far detectors [SK, ...] are able to measure the interactions with much better 4$\pi$ efficiency. Moreover, bar-based scintillator trackers, offer very limited information to tracking algorithms to successfully reconstruct events with multiple tracks given that the information of two tracks crossing the same bar is merged. In the case of neutrino interactions with low-energy transfer to the nucleus most of the times the only final state particle is a lepton, which can be successfully identified. However, more complex topologies involving one or more hadrons in the final state have insufficient selection efficiencies and purities limiting the analysis to be mainly focused on low energy transfer neutrino interactions. 

In order to overcome this limitations and improve neutrino-nucleus cross-section understanding and neutrino oscillation measurements future analysis require a new detector concept capable to work with full angular acceptance and able to provide accurate tracking information such that events with multiple and short tracks can be successfully reconstructed.

% \begin{figure}[htb]
%     \centering
% %    \begin{tabular}{cc}
% 		\includegraphics[width=0.7\linewidth]{plots/CubeGEANT4.png}
% %	\end{tabular}
% 	\caption{Geometry of a single SuperFGD cube.}
%     \label{fig:cube3d}
% \end{figure}

To achieve this, a novel detector concept, SuperFGD, has been purposed and its under development~\cite{Blondel_2018}. It is a 3D array of 192$\times$56$\times$184 cubes, instead of bars, of 1$\times$1$\times$1\,cm$^3$ made of plastic scintillator as the one in Figure~\ref{fig:cube3d}. Each cube is intersected by three orthogonal wavelength-shifting (WLS) fibers collecting the scintillation light. The fine granularity of the cubes, together by the three complementary 2D planes information is expected to provide information that allows to reconstruct the event in 3D, such that 3D tracking techniques can separate and identify multiple tracks propagating at an arbitrary angle. 

For this technology to succeed however there are two caveats to overcome. 
\begin{itemize}
\item In one hand 2D to 3D plane matching introduces a number of geometrical ambiguities that fake real signals. If the measurements associated to this fake signals however follow some distribution different to that of real signals, an algorithm can be designed to tag them. 
\item In the other hand the fabrication of large number of cubes for this technology with perfect opacity is very challenging. Hence, the migration of light from one cube to its neighbors broadens the signals threatening its fine granularity. Moreover, thicker signals, create a much larger set of ambiguities significantly increasing the amount of fake signals.
\end{itemize}

In order to extract full potential of this detector, hence, a classification tool able to remove fake signals and reduce the tracks thickness as a pre-step or input data to future tracking algorithms is requiered. 
